On the Efficiency of NLP-Inspired Methods for Tabular Deep Learning

Recent advancements in tabular deep learning (DL) have led to substantial performance improvements, surpassing the capabilities of traditional models. With the adoption of techniques from natural language processing (NLP), such as language model-based approaches, DL models for tabular data have also grown in complexity and size. Although tabular datasets do not typically pose scalability issues, the escalating size of these models has raised efficiency concerns. Despite its importance, efficiency has been relatively underexplored in tabular DL research. This paper critically examines the latest innovations in tabular DL, with a dual focus on performance and computational efficiency. The source code is available at https://github.com/basf/mamba-tabular.

==> encodings.tex <==

\begin{figure}[ht]
\centering
\begin{tikzpicture}[
    node distance=0.2cm and 0.5cm, % Reduced node distances for closer elements
    feature/.style={draw, thick, rectangle, fill=yellow!20, minimum width=1.5cm, minimum height=0.5cm},
    arrow/.style={-Stealth, thick},
    block/.style={draw, rounded corners, thick, fill=gray!10, text width=1.2cm, align=center, minimum height=1cm},
    matrixstyle/.style={matrix of nodes, nodes={draw, minimum size=5mm, fill=yellow!20}, column sep=1mm, row sep=1mm, nodes in empty cells},
    transformer/.style={draw, rounded corners, thick, fill=gray!10, text width=1.2cm, align=center, minimum height=1cm, rotate=90},
]

% Numerical features vector
\matrix (numFeatures) [matrixstyle, label=left:$x_{num}$] {
    \\
    \\
    \\
};

% Categorical features vector
\matrix (catFeatures) [matrixstyle, below=of numFeatures, label=left:$x_{cat}$, nodes={fill=red!20}] {
    \\
    \\
};

% Basis Expansion Block
\node[block, right=of numFeatures-2-1, yshift=-0.3cm] (basis) {\small{Encoder}};

% Feature matrix after basis expansion
\matrix (numFeatureMatrix) [matrixstyle, right=of basis, label=above: Encoded $x_{num}$] {
    & & &\\
    & & &\\
    & & &\\
};

\node[transformer, right=of numFeatureMatrix, xshift=-0.75cm, yshift=-0.3cm](numtok){\small Embedder};

\node[block, right=of catFeatures, xshift=-0.1cm, yshift=0cm] (tokenizer) {\small Encoder};
\node[transformer, right=of numFeatureMatrix, xshift=-2.3cm, yshift=-0.3cm] (cattok) {\small Embedder};

% All features matrix with CLS token
\matrix (allFeatures) [matrixstyle, right=of numtok, yshift=-1.5cm, xshift=0.5cm, nodes={fill=none}] {
    |[fill=yellow!20]| & |[fill=yellow!20]|& |[fill=yellow!20]|& |[fill=red!20]|&|[fill=red!20]|\\
    |[fill=yellow!20]| & |[fill=yellow!20]|& |[fill=yellow!20]|& |[fill=red!20]|&|[fill=red!20]|\\
    |[fill=yellow!20]| & |[fill=yellow!20]|& |[fill=yellow!20]|& |[fill=red!20]|&|[fill=red!20]|\\
    |[fill=yellow!20]| & |[fill=yellow!20]|& |[fill=yellow!20]|& |[fill=red!20]|&|[fill=red!20]|\\
    \node[draw=none] {$\vdots$}; & \node[draw=none] {$\vdots$}; & \node[draw=none] {$\vdots$}; & \node[draw=none] {$\vdots$}; & \node[draw=none] {$\vdots$}; \\
    |[fill=yellow!20]| & |[fill=yellow!20]|& |[fill=yellow!20]|& |[fill=red!20]|&|[fill=red!20]|\\
};

\draw [decorate, decoration={brace, amplitude=7pt, raise=2pt}]
    (allFeatures-1-5.north east) -- (allFeatures-6-5.south east) 
    node [midway, right=12pt, anchor=north, rotate=90] {$N$};

% Adding curly brackets with text above the first row
\draw [decorate, decoration={brace, amplitude=7pt, raise=2pt}] 
    (allFeatures-1-1.north west) -- (allFeatures-1-5.north east) 
    node [midway, yshift=0.6cm] {$\times J$}
    node [midway, yshift=1.1cm] {\footnotesize{Pseudo seq-length}};


\draw [decorate, decoration={brace, amplitude=8pt, raise=18pt, mirror}] 
    (allFeatures-6-1.north west) -- (allFeatures-6-3.north east) 
    node [midway, yshift=-1.2cm] {$\textbf{z}_{num}$}
    node [midway, yshift=-1.7cm, xshift=0.6cm] {$\in \mathbb{R}^{N\times J \times d}$};


    

\draw [decorate, decoration={brace, amplitude=8pt, raise=18pt, mirror}] 
    (allFeatures-6-4.north west) -- (allFeatures-6-5.north east) 
    node [midway, yshift=-1.2cm] {$\textbf{z}_{cat}$};

% Arrows from numerical features to basis expansion
\foreach \i in {1,2,3} {
    \draw[arrow] (numFeatures-\i-1) -- (basis);
}

% Arrows from basis expansion to numerical feature matrix
\draw[arrow] (basis) -- (numFeatureMatrix);

% Arrow from feature matrices to all features matrix
\draw[arrow] (numFeatureMatrix.east) -- (numtok.north);
\draw[arrow] (catFeatures.east) -- (tokenizer.west);
\draw[arrow] (tokenizer.east) -- (cattok.north);

\draw[arrow] (numtok.south) -- ([xshift=0.4cm]numtok.south);

\draw[arrow] (cattok.south) -- ([xshift=0.4cm]cattok.south);






\end{tikzpicture}
\caption{Generation of the input matrix that are fed through the Mamba blocks. The categorical features are tokenized and embedded similar to classical embeddings for language models. The numerical features are encoded and embedded via a simple linear layer. The final input matrix of the Mamba blocks are the concatenated embeddings  $\mathbf{z} \in \mathbb{R}^{N \times J \times d}$ with embedding dimension $d$.}
\label{fig:feature_processing}
\end{figure}




==> forward_pass.tex <==


\begin{figure}[ht]
\centering


\begin{tikzpicture}[
  node distance=0.4cm and 0cm,
  every node/.style={draw, very thick, rounded corners, minimum width=2.0cm, minimum height=0.9cm, align=center, font=\small},
  arrow/.style={->, thick},
  background rectangle/.style={fill=gray!20, rounded corners}
]

% Nodes
\node (input) [draw, fill=yellow!20] {Input Sequence $\mathbf{x}$};
\node (encoding) [ellipse, draw,minimum width=1.5cm, minimum height=1cm,  right=of input,  yshift=0.9cm, label=center:{Encoding}] {};
\node (embedding) [above=of input, yshift=0.25cm, draw, fill=yellow!20] {Embedding Layer};


\node (conv) [above=of embedding, draw, fill=red!20] {1D Convolution \\ Linear Layer};
\node (x_part) [above left=0.3cm and -0.3cm of conv, draw, fill=red!20, minimum height=0.5cm] {$\mathbf{z}$};
\node (z_part) [above right=0.3cm and -0.3cm of conv, draw, fill=red!20, minimum height=0.5cm] {$\mathbf{z'}$};

\node (A-matt) [above= of z_part, draw, fill=gray!20] {$\mathbf{A}$ \\ $\mathbf{B}$ \\ $\mathbf{\Delta}$};
\node (D-matt) [above= of A-matt, draw, fill=gray!20] {$\mathbf{\alpha}$ \\ $\mathbf{C}$};

\node (hidden_update) [above=of x_part, draw, fill=blue!20] {SSM};
\node (ssm) [ellipse, draw,minimum width=1.9cm, minimum height=1cm,  fill=blue!20, left=of hidden_update,  xshift=-0.5cm, yshift=0.0cm, label=center:{Update \\ Eq. 2}] {};
\node (elementwise_mult) [above=of hidden_update, draw, fill=green!20] {$\tilde{\mathbf{x}} = (\mathbf{H} \cdot \mathbf{C}^T) + \mathbf{\alpha} \odot \mathbf{z}$};
\node (linear) [above=of elementwise_mult, draw, fill=green!20, minimum height=0.9cm] {Linear Layer};
\node (Tabular head) [above=of input, yshift=7.8cm, draw, fill=red!20, minimum width=5.5cm,] {Tabular head};

% Mamba block
\begin{scope}[on background layer]
  \fill[gray!10, rounded corners, draw=black, very thick] ($(hidden_update.north west) + (-0.75, 3.0)$) rectangle ($(linear.south east) + (3.9, -5.2)$);
\end{scope}
\draw [decorate, decoration={brace, amplitude=10pt, raise=5pt}, thick] 
  ($(hidden_update.north east) + (3.9, 3.0)$) -- 
  ($(linear.south east) + (3.9, -5.2)$) 
  node[midway, xshift=1.2cm, yshift=-0.2cm, rotate=90, draw=none, minimum width=0cm, minimum height=0cm] {$N \times$ Mamba Block};



% Connections
\draw[arrow] (input) --  (embedding);
\draw[arrow] (encoding) -- ++(-2cm,0);
\draw[arrow] (embedding) -- (conv);
\draw[arrow] (conv) -- (x_part);
\draw[arrow] (conv) -- (z_part);
\draw[arrow] (x_part) -- (hidden_update);
\draw[arrow] (hidden_update) --  (elementwise_mult);
\draw[arrow] (elementwise_mult) -- (linear);
\draw[arrow] (D-matt) -- (elementwise_mult.east);
\draw[arrow] (hidden_update.west) -- (ssm.east);
\begin{scope}[on background layer]
  \draw[arrow, dashed] (z_part) -- (linear.east);
\end{scope}

\draw[arrow, bend right] (A-matt) to (hidden_update);
\draw[arrow] (x_part) to (A-matt);
%\draw[arrow] (hidden_update.north) to[out=120, in=180, looseness=5] (hidden_update.west);
\draw[arrow] (linear) to (Tabular head);


\end{tikzpicture}


\caption{The forward pass of a single sequence in the model. After embedding the inputs, the embeddings are passed to several Mamba blocks. The tabular head is a single task specific output layer. Before being passed to the Linear Layer, the contextualized embeddings are pooled via average pooling. For bidirectional processing a second block with a flipped sequence is used and the learnable matrices are not shared between the directions.}
\label{fig:forward_pass}
\end{figure}




==> mamba_arch.tex <==
\begin{figure}[ht]
\centering
\begin{tikzpicture}
    \tikzset{
        box/.style={rectangle, draw, minimum width=1.1cm, minimum height=1.1cm, rounded corners, thick},
        arrow/.style={-Stealth, thick},
        dashedarrow/.style={-Stealth, thick, dashed},
        input/.style={rectangle, draw=none, fill=none, text=red, minimum width=1.5cm},
        output/.style={rectangle, draw=none, fill=none, text=purple, minimum width=1.5cm}
    }

    % Nodes
    \node[box, shading=axis, left color=yellow!20, right color=red!30] (x) {$z_j$};
    \node[box, right=of x, fill=gray!10] (B) {$B$};
    \node[box, right=of B, fill=blue!20] (h) {$h_j$};
    \node[box, below=of h, fill=blue!20, node distance=2cm] (A) {$A h_{j-1}$};
    \node[box, right=of h, fill=gray!10] (C) {$C$};
    \node[box, fill=green!20, right=of C] (y) {$\tilde{x}_j$};
    \node[box, above=of h, fill=gray!10, node distance=2cm] (D) {$\mathbf{\alpha}$};

    % Arrows
    \draw[arrow] (x) -- (B);
    \draw[arrow] (B) -- (h);
    \draw[arrow] (h) -- (C);
    \draw[arrow] (C) -- (y);
    
    % Curved arrows for recursive update
    \draw[arrow] (h.west) to[out=225, in=135] (A.west);
    \draw[arrow] (A.east) to[out=45, in=-45] (h.east);

    % Curved arrows to and from D
    \draw[arrow] (x.north) to[out=45, in=180] (D.west);
    \draw[arrow] (D.east) to[out=0, in=135] (y.north);

    % Dotted curved arrows
    \draw[dashedarrow] (x.south) to[out=-45, in=-135] (B.south);
    \draw[dashedarrow] (x.north) to[out=15, in=155] (C.north);

\end{tikzpicture}
\caption{SSM updating step with recursive update of $h$: The hidden state is iteratively updated by going through the sequence (features) similar to a recurrent neural network. The final representation is generated as described in Equations 3-4.}
\label{fig:mamba_arch}
\end{figure}


==> old_tables.tex <==

\begin{table}[h!]
\centering
\begin{tabular}{l|ccccc}
\hline
\textbf{Model} & CPU & DI & HS & AB & CA \\
\hline
xgb & \textbf{0.024} \std{0.004} & 0.019 \std{0.001} & \textbf{0.113} \std{0.020} & 0.505 \std{0.030} & 0.174 \std{0.008} \\
FT & 0.034 \std{0.005} & 0.020 \std{0.001} & 0.151 \std{0.038} & 0.458 \std{0.021} & 0.185 \std{0.005} \\
MLP & 0.033 \std{0.003} & 0.064 \std{0.001} & 0.155 \std{0.021} & 0.472 \std{0.026} & 0.204 \std{0.008} \\
ResNet & 0.031 \std{0.004} & 0.030 \std{0.013} & 0.135 \std{0.016} & 0.463 \std{0.017} & 0.187 \std{0.010} \\
TabTransformer & - \std{0.001} & 0.022 \std{0.001} & 0.172 \std{0.031} & 0.468 \std{0.030} & 0.202 \std{0.008} \\
\hline
Mambular  & 0.027 \std{0.003} & 0.019 \std{0.001} & 0.114 \std{0.025} & 0.454 \std{0.024} & 0.169 \std{0.008} \\
Mambular$^b$ & 0.028 \std{0.004} & 0.019 \std{0.001} & 0.118 \std{0.026} & 0.454 \std{0.029} & \textbf{0.167} \std{0.008} \\
Mambular$^{b}_i$&  0.028 \std{0.002} & \textbf{0.018} \std{0.001} & 0.115 \std{0.031} & 0.450 \std{0.026} & 0.171 \std{0.007} \\
Mambular$_i$ & 0.029 \std{0.004} & 0.019 \std{0.001} & 0.118 \std{0.034} & \textbf{0.445} \std{0.020} & 0.169 \std{0.009} \\
\bottomrule
\end{tabular}
\caption{MSE Scores with Standard Deviations}
\end{table}



\begin{table}[]
    \centering
    \begin{tabular}{l|cccc|ccccc}
        \toprule
        \textbf{Model} & AD & FI & CH & BA & CPU & DI & HS & AB & CA\\
        \hline
        Mambular & \textbf{0.927} & 0.792  & 0.858  & 0.918 & \textbf{0.027} & 0.019  & 0.114  & 0.454 & 0.169  \\
        Mambular$^b$ & 0.926  & \textbf{0.793} & 0.861 & \textbf{0.920}  & 0.028  & 0.019  & 0.118  & 0.454  & \textbf{0.167}  \\
        Mambular$^{b}_i$ & 0.926 & 0.791  & \textbf{0.862} & 0.919 &  0.028 & \textbf{0.018}  & 0.115 & 0.450  & 0.171  \\
        Mambular$_i$ & 0.926  & 0.792  & 0.859  & 0.919 & 0.029  & 0.019  & 0.118  & \textbf{0.445}  & 0.169 \\
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}

\begin{table}[h!]
\centering
\begin{tabular}{l|cccc}
\hline
\textbf{Model} & AD& FI & CH & BA \\
\hline
xgb & \textbf{0.929} \std{0.002} & 0.774 \std{0.009} & 0.845 \std{0.008} & \textbf{0.928} \std{0.004} \\
FT & 0.925 \std{0.002} & 0.793 \std{0.010} & 0.858 \std{0.004} & 0.922 \std{0.004} \\
MLP & 0.913 \std{0.002} & 0.793 \std{0.012} & 0.841 \std{0.006} & 0.894 \std{0.005} \\
ResNet & 0.916 \std{0.003} & \textbf{0.794} \std{0.012} & 0.842 \std{0.007} & 0.898 \std{0.004} \\
TabTransformer & 0.920 \std{0.002} & - & 0.849 \std{0.006} & 0.926 \std{0.005} \\
\hline
Mambular & 0.927 \std{0.002} & 0.792 \std{0.012} & 0.858 \std{0.006} & 0.918 \std{0.004} \\
Mambular$^b$ & 0.926 \std{0.002} & 0.793 \std{0.012} & 0.861 \std{0.005} & 0.920 \std{0.003} \\
Mambular$^{b}_i$& 0.926 \std{0.003} & 0.791 \std{0.012} & \textbf{0.862} \std{0.006} & 0.919 \std{0.004} \\
Mambular$_i$ & 0.926 \std{0.002} & 0.792 \std{0.013} & 0.859 \std{0.005} & 0.919 \std{0.004} \\
\bottomrule
\end{tabular}
\caption{AUC Scores with Standard Deviations}
\end{table}



\begin{table}
    \centering
    \begin{tabular}{l|ccccc}
    \toprule
         Models &  CPU & DI & HS & AB & CA\\
         \hline
         Mambular& 0.027 \std{0.003}  & 0.019 \std{0.0011} & 0.114 \std{0.025} & \textbf{0.454}\std{0.024} & 0.169 \std{0.008}\\
         XGB & 0.024 \std{0.004}        & 0.019 \std{0.0013} & 0.113 \std{0.020} & 0.505 \std{0.030} &  0.174 \std{0.008}\\
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}


\begin{table}
    \centering
    \begin{tabular}{l|cccc}
    \toprule
         Models & AD & FI & CH & BA \\
         \midrule
         Mambular & 0.927\std{0.002} & \textbf{0.792}\std{0.012} & \textbf{0.858}\std{0.006} & 0.919\std{0.004} \\
         XGB      & \underline{0.929}\std{0.002} & 0.774\std{0.009} & 0.845\std{0.008} & \textbf{0.928}\std{0.004} \\
    \bottomrule
    \end{tabular}
    \caption{Performance metrics (AUC and accuracy) for different models across datasets.}
    \label{tab:my_label}
\end{table}



\begin{table}[H!]
    \centering
    \begin{tabular}{l|ccccc|cccc}
    \toprule
          Models   &  CPU $\downarrow$& DI $\downarrow$& HS $\downarrow$& AB $\downarrow$& CA $\downarrow$& AD $\uparrow$& FI $\uparrow$& CH $\uparrow$& BA $\uparrow$\\
          \hline
          Mambular & 0.027  & 0.019 & 0.114& \textbf{0.454} & 0.169  & 0.927 & \textbf{0.792} & \textbf{0.858} & 0.919 \\
          XGB      & 0.024  & 0.019 & 0.113  & 0.505  &  0.174  & \underline{0.929} & 0.774& 0.845 & \textbf{0.928} \\
          \bottomrule
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}
